TreeMind: Automatically Reproducing Android Bug Reports via LLM-empowered Monte Carlo Tree Search

Automatically reproducing Android app crashes from textual bug reports is challenging, particularly when the reports are incomplete and the modern UI exhibits high combinatorial complexity. Existing approaches based solely on reinforcement learning or large language models (LLMs) exhibit limitations in such scenarios. They struggle to infer unobserved steps and reconstruct the underlying user action sequences to navigate the vast UI interaction space, primarily due to limited goal-directed reasoning and planning. We present TreeMind, a novel technique that integrates LLMs with an adapted Monte Carlo Tree Search (MCTS) algorithm to achieve strategic UI exploration in bug reproduction. To the best of our knowledge, this is the first work to combine external decision-making with LLM semantic reasoning for reliable and accurate reproduction processes. We formulate the reproduction task as a target-driven search problem, leveraging MCTS as the core planning mechanism to iteratively refine action sequences. To enhance MCTS with semantic reasoning, we introduce two LLM-guided agents with distinct roles: Expander generates top-k promising actions based on the current UI state and exploration history, while Simulator estimates the likelihood that each candidate action leads toward successful reproduction by additionally leveraging dynamic environment feedback. By incorporating multi-modal UI inputs and tailored prompting strategies, TreeMind performs feedback-aware navigation that identifies essential user actions and incrementally reconstructs reproduction paths. We evaluate TreeMind on a dataset of 93 real-world Android bug reports from three widely-used benchmarks. Experimental results show that it significantly outperforms four state-of-the-art baselines, including ReBL, ReActDroid, AdbGPT, and ReproBot, in reproduction success rate.

==> mainBody/mcts.tex <==
%!TEX root = sample-acmsmall-conf.tex

\newpage
\subsection{LLM-assisted Monte Carlo Tree Search}

We integrate an LLM-based multi-agent framework with MCTS to enable effective exploration in the complex state space of bug reproduction.
This integration forms a closed-loop and feedback-driven process, where the agents provide semantic guidance while MCTS drives goal-directed exploration in the large and sparse state space. 
By leveraging incremental feedback, the agents dynamically refine their understanding of the crash scenario and adapt the exploration strategy, making \oursystem well-suited for bug reports with incomplete or ambiguous reproduction steps.

To operationalize this integration, we introduce LLM-based agents in the expansion and simulation stages of MCTS, where semantic reasoning and adaptive decision-making are essential.
In contrast, the selection and backpropagation, which primarily involve numerical computations, are handled without LLMs.
Instead, we make task-specific modifications to the underlying algorithms in these two stages to better support the requirements of bug reproduction.
We now describe each of the four stages in detail.

\subsubsection{Selection}
Starting from the root node representing the initial UI state, we follow a path in the Monte Carlo Tree by recursively selecting child nodes based on exploration heuristics.
In our task setting, where the environment consists of high-branching UI states and delayed rewards, the standard Upper Confidence Bound (UCB)~\cite{auer2002nonstochastic} used in the stage may lead to over-exploitation of early promising paths and insufficient exploration of alternative states.
To address this, we adopt a variant known as the Softmax-over-UCB strategy, which assigns selection probabilities to available child nodes according to their UCB scores.
This approach transforms deterministic UCB scores into a probability distribution using a softmax function, enabling stochastic yet guided selection.
This design encourages exploration of underexplored areas while still favoring high-reward nodes, thereby improving state space coverage and mitigating premature convergence.

Given a set of child nodes with UCB scores $\{u_1, u_2, ..., u_n\}$, the selection probability for the $k$-th node in the tree is computed as:

\begin{equation}
P(k) = \frac{e^{\lambda u_k}}{\sum_{j=1}^n e^{\lambda u_j}},\,\text{where}\,\,\,u_k = R_k + c\sqrt{\frac{\ln N}{n_k}}
\end{equation}
, where $R_k$ is the empirical mean reward of the node, $n_k$ is the number of times the node has been selected, $N$ is the total number of visits to the parent node, $c$ is an exploration coefficient controlling the trade-off between exploration and exploitation, and $\lambda$ is a temperature parameter that adjusts the sharpness of the softmax distribution.

At each search iteration, TreeMind computes UCB scores for all expanded child nodes of the current node and samples one according to the resulting softmax probabilities.
This selection process repeats recursively, until a leaf node or an unexpanded node is reached. 
At that point, the algorithm transitions into the expansion stage.

\subsubsection{Expansion}
This stage adds new nodes to the search tree, enabling exploration of alternative paths.
However, traditional MCTS expands only a single node per iteration, which can hinder effective UI exploration in the scenario of bug reproduction.
Such scenario often involves noisy feedback and high branching factors, often exacerbated by incomplete bug reports that provide limited guidance for the search.
As a result, early reward signals may not accurately reflect true progress, causing the algorithm to prematurely commit to misleading paths while the correct reproduction sequence remains hidden in unexplored branches.

\noindent\textbf{Expander Agent.} We introduce Expander, an LLM-based agent designed to assist the expansion stage of MCTS by selecting a small number of promising child nodes for further exploration.
Instead of expanding a single child node per iteration, the agent is responsible for performing a top-\textit{k} expansion strategy based on the LLM's ranking of candidate actions, enabling broader yet focused exploration.
At each expansion step, Expander queries the LLM using the \textit{ExpansionPrompt} defined earlier (Section \red).
The LLM uses its reasoning ability to estimate how likely each candidate action is to advance toward the reproduction goal, based on semantic cues from the bug report and the exploration history.
It then returns a ranked list of candidate actions, from which the top-\textit{k} are selected to the search tree to enable broader exploration.

The expansion strategy enhances exploration diversity by allowing the search to pursue multiple promising directions simultaneously, rather than being constrained to a single path.
This reduces the risk of getting trapped in misleading paths caused by noisy feedback.
Broadening the exploration frontier makes \oursystem more robust to the uncertainty and partial information typical of real-world bug reports.
This, in turn, increases the likelihood of reaching a correct reproduction path.

\subsubsection{Simulation}
At this stage, \oursystem estimates the potential of each expanded candidate action to contribute to a successful reproduction, providing a value signal to guide subsequent decision-making in the search process.
The bug reproduction often demands extended sequences of UI interactions, where each step presents many possible actions.
This combination of long paths and high branching factors results in an intractably large search space, making it unrealistic to simulate every candidate action within a reasonable time frame.

\noindent\textbf{Simulator Agent.} We design an LLM-based agent named Simulator, which performs lightweight simulation by estimating the potential of each candidate action without executing full interaction paths.
For each candidate action, the Simulator executes it in the runtime environment using the Action Execution Engine, and observes the resulting UI transitions.
For each observed UI transition, the agent invokes an LLM to evaluate its semantic relevance to the expected behavior depicted in the input bug report, while also considering the execution context accumulated along the current path on the search tree.
With this relevance, the agent estimates the effectiveness of each action in driving the exploration toward successful crash reproduction, and assigns a heuristic score that reflects its utility in the search process.

To ensure independent simulation of each action, \oursystem employs an app state recovery mechanism. 
After simulating an action, it restores the app to the state of the parent node, ensuring that each subsequent simulation starts from a consistent state.
During each expansion, \oursystem records the selected action in the search tree node and maintains the full action sequence from the root to the current node, capturing the interaction history that leads to the current UI state.
This design allows \oursystem to restart the app from a clean state and replay the recorded actions to accurately reconstruct the associated UI.

\subsubsection{Backpropagation}
Both the heuristic scores and visit counts are incrementally updated along the path from the expanded node to the root at this stage.
If a node expands into \textit{k} child nodes, their scores are aggregated and normalized by averaging, in order to prevent score inflation caused by a large number of children.
This normalization ensures that nodes with many low-quality children do not gain an unfair advantage in subsequent selection.
Each node accumulates the normalized score by adding it to its existing total score, allowing the value to reflect aggregated feedback over multiple simulations.
By propagating the normalized score up the tree, \oursystem maintains balanced and stable value estimates across different paths, supporting robust exploration and evaluation.

==> mainBody/prompt_design.tex <==
\subsection{Prompt Design}\label{sec:sign}
Prompt engineering plays a crucial role in enabling LLM-based agents to understand contextual information and effectively reproduce bugs in Android apps.
Existing techniques have proposed various prompts for bug reproduction~\cite{wang2024feedback,feng2024prompting,huang2025one}.
However, these prompts cannot be directly applied to our work, since they are not designed to integrate with external planning strategies, which are crucial for effective UI state space exploration.

% However, these prompts are not directly applicable to our work, because existing prompts are not designed to integrate LLMs with external planning strategies, which limits their ability to support effective UI state space exploration.
% (1) They do not consider the integration of LLMs with external planning strategies, which in turn hinders effective state space exploration.
% (2) They primarily focus on prompting a single LLM to perform the task, without considering role specialization among multiple LLM-based agents.

To overcome the limitation, we design two sets of role-specific prompts, \ie, ExpandPrompt and SimulatePrompt listed in \Cref{tab:prompt1}, to enable seamless integration of general-purpose LLMs into our framework.
% draw inspiration from the prompt design of ReBL ~\cite{wang2024feedback} and 
These prompts instantiate LLMs as domain-aware agents, aligned with the expansion and simulation stages of the MCTS process, respectively.
The interaction between these agents and the core search mechanism of MCTS is described in the later section.
% Specifically, these prompts transform LLMs into domain-aware agents with distinct roles, where ExpPrompt is aligned with the expansion stage, and SimPrompt with the simulation stage in the MCTS process.
% each tailored to perform subtasks, such as interpreting bug reports or generating candidate actions.
To improve the agents’ ability to perform complex tasks and support downstream decision-making, we apply advanced prompt engineering techniques, namely few-shot learning~\cite{liu2023pre} and chain-of-thought reasoning~\cite{wei2022chain}.
These techniques not only enable LLMs to perform modular task decomposition and multi-step reasoning, but also provide structured instructions and ensure consistent output formatting.

\input{mainBody/table/prompt}
\subsubsection{Task Specification}
While LLMs possess general reasoning capabilities, they often lack the task-specific focus required for effective bug reproduction.
We design role-specific instructions that specialize LLMs into dedicated agents aligned with our overall workflow. 
% These instructions also enforce a predefined output schema to ensure consistency and facilitate downstream integration.
As listed in the second row of \Cref{tab:prompt1}, we adopt prompt engineering strategies tailored to each agent’s responsibilities, enabling general LLMs to emulate the behavior of different experts for automated bug reproduction.
% These prompts clearly define the operational context, expected outputs, and reasoning objectives for each role.
% clearly defining its operational context and expected outputs.
% This setup enables the LLM to reason within the appropriate domain, follow established conventions, and consistently generate outputs that conform to the required schema across diverse reproduction scenarios.

The motivation prompts are designed to clearly define the LLM’s roles and objectives, guiding its behavior in the reproduction task.
They explicitly instruct LLMs not only to execute the reproduction steps, but also to observe and confirm whether the specific buggy behavior described in the input report is actually triggered.
This clear goal enhances both the reliability and accuracy of the reproduction process.
For example, in the ExpandPrompt, we design a motivation prompt aimed at transforming the LLM into an expert in bug reproduction, enabling it to generate the most plausible actions for reproducing the bugs. Moreover, in the SimulatePrompt, the motivation prompt guides the LLM to evaluate the target step with greater accuracy and domain-specific expertise, effectively transforming it into a professional scorer.
% The motivation prompt defines the LLM’s role and objectives, transforming it into an expert agent for bug reproduction. 
% It instructs the model not only to follow reproduction steps but also to observe and confirm that the exact buggy behavior described in the report is triggered. 
% By establishing this clear goal, the prompt guides the LLM to focus on both procedural correctness and behavioral validation, improving the reliability and accuracy of automated reproduction.

To help the LLM-based agents effectively interpret the environment, we provide a well-structured input specification that encodes both textual and visual information about the app and its UI.
Specifically, the input includes the app name, the textual bug report, a structured description of the explored UI components, and the current UI screenshot.
This multi-modal input enables LLMs to better understand the screen’s functional layouts and their spatial relationships, disambiguate similarly named elements, and accurately associate bug descriptions with on-screen components.
By explicitly presenting this information, the input forms a solid foundation for precise and context-aware action generation.

% By aligning the structured textual descriptions with the corresponding visual information, \oursystem allows the LLM to reason over both semantic and visual modalities, enabling it to identify functional relationships between UI components, disambiguate similarly named elements, and interpret unconventional layouts. By explicitly presenting this information, the LLM can accurately interpret and incorporate it into its reasoning process, forming a foundation for precise action generation.

% By presenting this information in a consistent and interpretable format, the input specification forms a reliable foundation for the LLM’s reasoning and decision-making throughout the reproduction process.




% To ensure that the LLM clearly understands the types of information it receives, the input specification module provides structured app-related data, including the app name, bug report text, a description of the current screen layout and state. Moreover, to enhance the LLM’s comprehension of UI semantics and spatial arrangements, \oursystem adopts a multi-modal UI representation that combines the UI grouping technique introduced by ReBL with pixel-level UI screenshots.
% By aligning the structured textual descriptions with the corresponding visual information, \oursystem allows the LLM to reason over both semantic and visual modalities, enabling it to identify functional relationships between UI components, disambiguate similarly named elements, and interpret unconventional layouts. By explicitly presenting this information, the LLM can accurately interpret and incorporate it into its reasoning process, forming a foundation for precise action generation. 

To ensure deterministic parsing and minimize ambiguity, we enforce a structured output format across all prompts. 
This guarantees consistent communication with downstream components and significantly reduces integration errors from verbose or inconsistent outputs.
For the ExpandPrompt, inspired by the action format in ReBL, we restrict the output to 6 predefined actions: click, long-click, set-text, multiple-select, rotate, and back.
For example, in the ExpandPrompt, the LLM is required to return the action list in a strict JSON-like format, as illustrated in \Cref{tab:prompt1}, namely: Your suggestions should be formatted as follows: [\{'action': 'x1', 'feature': 'y1'\}, \{'action': 'x2', 'feature': 'y2'\}, ...]. For the SimulatePrompt, LLMs are prompted to output a numerical score in a fixed format, constrained to the range [0, 10].
This ensures compatibility with the backpropagation stage in MCTS.


% Specifically, to ensure deterministic parsing and minimize ambiguity, we enforce a structured output format across all prompt templates, which guarantees consistent communication with downstream components and significantly reduces integration errors caused by verbose or inconsistent outputs. For the ExpandPrompt, inspired by the action format in ReBL~\cite{wang2024feedback}, we define restrictive rules for 6 supported actions: click, long-click, set-text, multiple-select, rotate, and back. The LLM's final output should obey the format rule shown in the output restriction fild. For the SimulatePrompt, as listed in \Cref{tab:prompt}, the LLM is instructed to output a numerical score in a fixed format, with its value constrained to the range [0,10]. This ensures compatibility with the backpropagation stage in MCTS.
%This design choice guarantees consistent communication with downstream components and significantly reduces integration errors caused by verbose or inconsistent outputs.
% \oursystem employs role-specific prompt engineering to define the LLM’s operational context, responsibilities, and output requirements. 
% These predefined instructions guide the model to exhibit domain-specific reasoning, follow established conventions, and produce format-compliant results across various reproduction scenarios.

% Specifically, we adopt a structured prompting approach based on ReBL, which explicitly defines the task objective, outlines the workflow, and provides a comprehensive explanation to guide the LLM’s behavior.
% With this specification, \oursystem is capable of performing

% This section presents the instruction design in \oursystem, which adapts a general-purpose LLM into a domain-specialized agent for Android crash reproduction while ensuring that outputs follow a predefined schema.

% \textit{1) Task Specification:}

% While LLMs possess general capabilities, they lack the task-specific focus required for bug reproduction.
% Therefore, we leverage task-specific instructions for the task specification to effectively specialize the LLM into a dedicated agent, guiding its behavior in alignment with our overall workflow.
% Specifically, we adopt a structured prompting approach based on ReBL, which explicitly defines the task objective, outlines the workflow, and provides a comprehensive explanation to guide the LLM’s behavior.
% With this specification, \oursystem is capable of performing



%\subsubsection{Response Restriction}
% To enable deterministic parsing and reduce ambiguity, \oursystem enforces a structured output format in both prompt sets. This ensures consistent integration with downstream modules and minimizes errors from inconsistent or verbose responses.

%To ensure deterministic parsing and minimize ambiguity, we enforce a structured output format across all prompt templates.
%This design choice guarantees consistent communication with downstream components and significantly reduces integration errors caused by verbose or inconsistent outputs.

%As listed in \red,
%For the ExpandPrompt, inspired by the action format in ReBL~\cite{wang2024feedback}, we define restrictive rules for 6 supported actions: click, long-click, set-text, multiple-select, rotate, and back.
%To facilitate integration with the expansion stage in the MCTS subsequently, we require the LLM to produce a fixed number of candidate actions in a single response.

% \textcolor{red}{To improve efficiency during the MCTS expansion phase, \oursystem uses a \textit{top-k} strategy that allows the LLM to generate multiple candidate actions in a single response, reducing the number of calls and accelerating exploration.}

% For the SimulatePrompt, as listed in \red, the LLM is instructed to output a numerical score in a fixed format, with its value constrained to the range [0,10]. This ensures compatibility with the backpropagation stage in MCTS.

% In the simulation phase, simulator outputs a numerical score in a fixed format, ensuring compatibility with the subsequent backpropagation step in MCTS.


\subsubsection{Few-shot learning}
% Carefully designed few-shot examples are embedded directly into each prompt as in-context demonstrations. 
% The ExpandPrompt guides the model in converting bug report descriptions into structured action sequences with the correct format.
% The SimulatePrompt instructs the model to evaluate these sequences by estimating their likelihood of reproducing the crash and assigning schema-compliant scores.
Each prompt embeds carefully crafted in-context examples. 
The ExpandPrompt guides LLMs in converting bug descriptions into structured action sequences, while the SimulatePrompt instructs LLMs to evaluates the likelihood of reproducing the bug based on the sequences and assigns schema-compliant scores.

As shown in the the third row of \Cref{tab:prompt1}, the few-shot examples are carefully selected to span a wide range of scenarios, enabling prompts to elicit expert-level behavior from the outset.
% For instance, the second row in \Cref{tab:prompt1} illustrates several representative examples. 
In the ExpandPrompt, the example demonstrates how to generate possible actions for bug reproduction and return them in the correct structured format.
Based on the bug report and the UI element grouping results, clicking \textit{`Profile'} appears to be a reasonable initial action for reproducing the bug. However, in some cases, multiple UI elements may share the same label. Consequently, the \textit{`Profile'} referenced in the bug report might be located on a different page. In such scenarios, it may also be reasonable to click \textit{`Settings'} or click \textit{`Home'} as alternative exploratory actions.

In the SimulatePrompt, the examples describe the process of scoring a target step, which provides critical guidance for determining the reproduction direction. In the first example, it is observed that the bug report exactly matches the target action, indicating that the target action should be assigned an extremely high score. In contrast, in the second example, a careful analysis reveals that the target action is likely to deviate the reproduction path from the correct trajectory; therefore, it should be assigned a low score.
Well-crafted exemplars guide LLMs’ decision-making and support generalization to novel but structurally similar inputs, leading to format-compliant outputs and more reliable MCTS-based search.

% All examples incorporate concise and well-structured reasoning steps, helping the LLM perform step-by-step reasoning.

% Learning from these exemplars helps LLMs generalize to novel but structurally similar inputs and produce format-compliant outputs, improving robustness to noisy bug reports and enhancing the reliability of the MCTS-based search.





% All examples incorporate carefully crafted reasoning steps, enabling the LLM to perform step-by-step reasoning and better  expert decision-making during the reproduction process.

% By imitating these exemplars, the model generalizes more effectively to novel but structurally similar inputs, producing outputs that are both semantically accurate and format-compliant. 

% This improves robustness to noisy bug reports and enhances the reliability of the MCTS-based search.

% Both agents are equipped with carefully crafted few-shot examples, which are embedded directly into their respective prompts to serve as in-context demonstrations. The examples guide the expander in decomposing bug report descriptions into structured action sequences, ensuring that each predefined action is produced in the correct format, while simultaneously instructing the simulator on evaluating these sequences, estimating their likelihood of reproducing the crash, and generating schema-compliant scores.

% These examples are deliberately selected to cover a diverse range of scenarios, enabling the agents to operate with expert-level proficiency from the outset. By observing and imitating these exemplars, the agents generalize more effectively to new but structurally similar situations, producing outputs that are both semantically accurate and format-compliant. This capability enhances robustness against noisy bug reports and strengthens the overall reliability of the MCTS-based search process.

\subsubsection{Chain-of-thought reasoning}
We adopt chain-of-thought (CoT) reasoning to elicit step-by-step reasoning, guiding LLMs to articulate intermediate steps explicitly and avoid errors from implicit assumptions or incomplete logic.
CoT also helps decompose complex tasks, enforce consistency, and resolve conflicting information, ultimately enhancing output reliability and interpretability in challenging bug reproduction scenarios.

% also helps decompose complex tasks, maintain consistency, and resolve conflicting information, improving both output reliability and interpretability in challenging bug reproduction cases.

As shown in the fourth row of \Cref{tab:prompt1}, CoT reasoning is used to guide LLMs through intermediate reasoning steps in a domain-specific bug reproduction case. 
For example, in the ExpandPrompt, we distill a set of reasoning strategies to guide the LLM in generating the most probable actions for successful bug reproduction. Similarly, we provide structured reasoning guidance for the LLM to evaluate and score target actions, enhancing both the accuracy and reliability of its scoring process.


\textcolor{red}{The prompt helps LLMs generate and evaluate candidate actions systematically, leading to a successful reproduction trace.
This enables TreeMind to navigate the MCTS search space more reliably in this instance.
\oursystem incorporates carefully crafted steps to guide the LLM in performing bug reproduction in a structured and domain-specific manner. By leveraging chain-of-thought reasoning, the LLM is able to approach the task through a structured, step-by-step reasoning process, systematically generating candidate actions, evaluating their potential outcomes, and refining its decisions based on intermediate reasoning. Ultimately, this mechanism enables \oursystem to effectively explore the search space during MCTS, guiding the reproduction process toward successful crash triggers with high reliability.}

% In order to improve decision-making accuracy, \oursystem incorporates chain-of-thought (CoT) reasoning as a core prompting strategy for both LLM-based agents. This approach guides the agents through a structured, step-by-step reasoning process, encouraging them to explicitly articulate intermediate inferences before arriving at a final decision. By externalizing the reasoning process, CoT reduces the likelihood of errors stemming from implicit assumptions, incomplete logical chains, or overlooked contextual constraints. Moreover, it enables the agents to more effectively decompose complex tasks, maintain consistency across multi-step operations, and reconcile conflicting pieces of information. The resulting transparency not only improves alignment between the agents’ actions and the target objectives but also enhances interpretability, making it easier to analyze and refine the agents’ decision-making strategies for challenging or ambiguous bug reproduction scenarios.

% Inspired by ReBL, we introduce a method to translate the LLM’s responses into concrete actions executed on the emulator using uiautomator2. Specifically, the action attribute in the LLM’s output corresponds to a single operation in uiautomator2, while the feature attribute identifies the target UI element. By invoking the function associated with the specified action on the designated UI element, uiautomator2 can seamlessly convert the LLM’s structured response into an executable operation on the emulator.

==> mainBody/table/baseline.tex <==
\begin{table}[ht]
    \centering
    \caption{Baseline Results}
    \label{tab:baseline}
    \resizebox{\linewidth}{!}{
    {\tiny
    
    \begin{tabular}{l|c c c c c|l|c c c c c}
    \toprule
        \textbf{Name} & \textbf{TM} & \textbf{RAD} & \textbf{ReBL} & \textbf{AdbGPT} & \textbf{RB} &
        \textbf{Name} & \textbf{TM} & \textbf{RAD} & \textbf{ReBL} & \textbf{AdbGPT} & \textbf{RB} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-6} \cmidrule(lr){7-7} \cmidrule(lr){8-12}
        TeamNewPipe-7825 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-25 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        sdbviewer-10 & 1:07.826 & 1:27.513 & 0:43.641 & $\times$ & $\times$ &
        recdroid-26 & 1:41.996 & 0:23.622 & $\times$ & $\times$ & $\times$ \\
        
        ankidroid-9914 & 14:08.895 & $\times$ & 4:18.445 & 4:47.051 & $\times$ &
        recdroid-27 & 3:34.568 & 0:59.017 & $\times$ & $\times$ & $\times$ \\
        
        ankidroid-10584 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-28 & 17:28.345 & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        fennifith-47 & 8:49.553 & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-29 & 2:57.714 & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        plusTimer-19 & 0:17.613 & 0:17.419 & 0:19.174 & 0:21.937 & 0:13.109 &
        recdroid-30 & 2:13.791 & $\times$ & 1:32.814 & 2:13.057 & 4:23.214 \\
        
        GrowTracker-89 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-31 & 2:54.398 & $\times$ & 2:41.760 & 2:31.891 & 3:17.593 \\
        
        timusus-456 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-33 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        ankidroid-3370 & 1:44.553 & 1:47.823 & $\times$ & 2:53.712 & $\times$ &
        recdroid-34 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        ankidroid-2765 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-35 & 9:53.310 & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        ankidroid-2564 & 1:03.786 & 0:51.749 & $\times$ & $\times$ & $\times$ &
        recdroid-38 & 0:13.680 & 0:16.188 & 0:01.757 & 0:07.314 & 0:19.251 \\
        
        ankidroid-2681 & 2:47.560 & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-39 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        cgeo-368 & 2:17.437 & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-42 & 9:13.038 & $\times$ & 1:17.487 & 2:12.583 & $\times$ \\
        
        tracker-55 & 1:07.129 & 2:37.106 & $\times$ & $\times$ & $\times$ &
        recdroid-45 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        GrowTracker-87 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-49 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        markor-1565 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-53 & 6:27.823 & $\times$ & 2:03.292 & 2:14.063 & $\times$ \\
        
        nRF-Mesh & 9:33.528 & 5:15.765 & $\times$ & $\times$ & 3:09.655 &
        recdroid-55 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        sdbviewer-7 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-56 & 2:17.731 & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        JonasBernard-30 & 3:41.243 & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-57 & 3:52.746 & $\times$ & 3:13.314 & $\times$ & $\times$ \\
        
        MCMrARM-183 & 23:50.998 & $\times$ & 9:36.157 & $\times$ & $\times$ &
        recdroid-58 & 1:15.350 & 0:24.272 & 0:47.112 & 1:17.243 & 9:37.431 \\
        
        ankidroid-3224 & 0:50.337 & $\times$ & $\times$ & $\times$ & $\times$ &
        recdroid-60 & 15:30.221 & 0:28.078 & $\times$ & $\times$ & $\times$ \\
        
        SecUSo--101 & 2:13.038 & 0:46.021 & $\times$ & $\times$ & $\times$ &
        recdroid-61 & 4:07.122 & 2:29.056 & $\times$ & $\times$ & 7:16.762 \\
        
        andror2-7 & 3:23.755 & 0:34.502 & 2:25.838 & $\times$ & $\times$ &
        recdroid-62 & 7:06.762 & $\times$ & 2:18.530 & $\times$ & $\times$ \\
        
        andror2-11 & 0:20.269 & 0:13.761 & 1:02.567 & 0:13.479 & $\times$ &
        recdroid-64 & 2.13.452 & 1:17.513 & 1:08.406 & $\times$ & $\times$ \\
        
        andror2-23 & 1:09.100 & 0:12.234 & 0:32.708 & 1:06.374 & 0:48.271 &
        saner2022-2 & 4:13.849 & 0:38.074 & $\times$ & $\times$ & 5:35.175 \\
        
        andror2-159 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        saner2022-8 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        andror2-162 & 2:01.675 & 0:52.817 & $\times$ & $\times$ & $\times$ &
        saner2022-11 & 0:02.559 & 0:13.025 & 0:02.879 & $\times$ & 0:40.559 \\
        
        andror2-164 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        saner2022-18 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        andror2-168 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        saner2022-23 & $\times$ & $\times$ & 1:58.626 & $\times$ & $\times$ \\
        
        andror2-198 & 1:32.610 & $\times$ & $\times$ & $\times$ & $\times$ &
        saner2022-129 & $\times$ & 1:42.512 & $\times$ & $\times$ & $\times$ \\
        
        andror2-276 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        saner2022-271 & $\times$ & $\times$ & 3:30.557 & $\times$ & $\times$ \\
        
        recdroid-1 & $\times$ & 0:45.041 & $\times$ & $\times$ & $\times$ &
        saner2022-1089 & 3:16.219 & 0:53.337 & 2:08.970 & 3.34.518 & 5:49.172 \\
        
        recdroid-2 & 4:17.318 & $\times$ & 2:31.865 & 2:18.704 & 3:14.211 &
        saner2022-1096 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        recdroid-3 & 2:06.807 & 0:40.967 & 1:06.807 & 2:06.173 & 1:49.194 &
        saner2022-1133 & 2:47.914 & $\times$ & 0:52.137 & 1:22.064 & 2:47.914 \\
        
        recdroid-5 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        saner2022-1160 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        recdroid-7 & 3:18.585 & 0:27.403 & 1:47.214 & 3:41.394 & 2:35.130 &
        saner2022-1207 & $\times$ & 1:24.699 & 1:57.485 & $\times$ & $\times$ \\
        
        recdroid-8 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        saner2022-1215 & 1:28.669 & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        recdroid-9 & 3:41.129 & $\times$ & 1:28.695 & $\times$ & 4:27.529 &
        saner2022-1227 & 17:33.244 & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        recdroid-11 & 0:34.988 & $\times$ & $\times$ & $\times$ & $\times$ &
        saner2022-1299 & $\times$ & 6:32.565 & $\times$ & $\times$ & $\times$ \\
        
        recdroid-12 & 1:55.505 & 0:25.406 & 1:26.284 & $\times$ & 2:18.074 &
        saner2022-1430 & $\times$ & 2:34.577 & $\times$ & $\times$ & $\times$ \\
        
        recdroid-13 & 2:34.317 & 0:33.679 & 1:31.550 & 2:19.057 & 1:16.385 &
        saner2022-1447 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        recdroid-14 & 3:33.467 & $\times$ & 0:50.672 & 4:11.409 & 2:58.417 &
        saner2022-1568 & $\times$ & 0:19.091 & $\times$ & $\times$ & $\times$ \\
        
        recdroid-15 & 5:44.074 & 0:40.742 & $\times$ & $\times$ & $\times$ &
        saner2022-1645 & $\times$ & $\times$ & 9:45.421 & $\times$ & $\times$ \\
        
        recdroid-17 & 1:07.909 & $\times$ & $\times$ & $\times$ & $\times$ &
        yakusu-1 & $\times$ & 1:22.458 & $\times$ & $\times$ & $\times$ \\
        
        recdroid-21 & 3:24.857 & $\times$ & 0:48.693 & $\times$ & $\times$ &
        yakusu-35 & 2:18.938 & $\times$ & $\times$ & $\times$ & $\times$ \\
        
        recdroid-23 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &
        yakusu-98 & 11:11.319 & $\times$ & $\times$ & $\times$ & 2:04.998 \\
        
        recdroid-24 & 4:39.605 & 0:23.204 & $\times$ & $\times$ & $\times$ & & & & &\\
        
    \bottomrule
    \end{tabular}
    }
    }
        % \caption*{111111111111}
\end{table}
